Observational Learning with a Budget

We consider a model of Bayesian observational learning in which a sequence of agents receives a private signal about an underlying binary state of the world. Each agent makes a decision based on its own signal and its observations of previous agents. A central planner seeks to improve the accuracy of these signals by allocating a limited budget to enhance signal quality across agents. We formulate and analyze the budget allocation problem and propose two optimal allocation strategies. At least one of these strategies is shown to maximize the probability of achieving a correct information cascade.

==> random_walk_fig.tex <==
\begin{figure}[h!]
\centering
\begin{tikzpicture}[scale=1.8]
\draw [decoration={markings,mark=at position 1 with {\arrow[scale=2,>=stealth]{>}}},postaction={decorate}] (0,0) -- (3.5,0);
\draw [decoration={markings,mark=at position 1 with {\arrow[scale=2,>=stealth]{>}}},postaction={decorate}] (3.5,0) -- (0,0);
\draw (1.75,0.05) -- (1.75,-0.05);
\draw (0.2,0.05) -- (0.2,-0.05);
\draw (3.3,0.05) -- (3.3,-0.05);
\node at (1.78,-0.17) {$0$};
\draw [->] (1.75,0) to [out=90,in=90] (2.05,0); \node at (1.92,0.2) {\scalebox{0.95}{$p_f$}}; \node at (2.05,-0.15) {$\eta$};
\draw [->] (2.05,0) to [out=90,in=90] (2.4,0); \node at (2.26,0.2) {\scalebox{0.95}{$p_f$}}; \node at (2.4,-0.15) {$2\eta$};
\draw [->] (1.75,0) to [out=-90,in=-90] (0.2,0); \node at (0.98,-0.3) {\scalebox{0.95}{$1-p_f$}};
\node at (0.10,-0.15) {$-1$};
\node at (3.3,-0.15) {$1$};
%\draw [->] (1.8,0) to [out=-90,in=-90] (0.3,0);
\end{tikzpicture}
\caption{\small Transition diagram of the random walk.}  
\label{random_walk}
\end{figure}

==> signal_channel_fig.tex <==
\begin{figure}[h!]
\centering
\begin{subfigure}{0.46\linewidth}
\centering
\begin{tikzpicture}[scale=1.4]
%%%%%%%%%%%%%%%%   BSC for receiving private signals    %%%%%%%%%
\draw [decoration={markings,mark=at position 1 with {\arrow[scale=2,>=stealth]{>}}},postaction={decorate}] (0,0) -- (1.5,0);
\draw [decoration={markings,mark=at position 1 with {\arrow[scale=2,>=stealth]{>}}},postaction={decorate}] (0,-1) -- (1.5,-1);
\draw [decoration={markings,mark=at position 1 with {\arrow[scale=2,>=stealth]{>}}},postaction={decorate}] (0,0) -- (1.5,-1);
\draw [decoration={markings,mark=at position 1 with {\arrow[scale=2,>=stealth]{>}}},postaction={decorate}] (0,-1) -- (1.5,0);
\node at (1.65,0) {$H$};
\node at (1.65,-1) {$L$};
\node at (-0.15,0) {$G$};
\node at (-0.15,-1) {$B$};
\node at (-0.35,-0.5) {$V$};
\node at (1.85,-0.5) {$S_i$};
\node at (0.75,0.15) {\scalebox{0.83}{$p$}};
\node at (0.75,-1.15) {\scalebox{0.83}{$p$}};
%\node at (0.4,-0.35) [rotate= -26.56] {$1-p$};
\node at (0.54,-0.22) [rotate= -33.7] {\scalebox{0.83}{$1-p$}};
\node at (0.56,-0.8) [rotate= 33.7] {\scalebox{0.83}{$1-p$}};
%\node at (0.8,-0.4) {$1-p$};
\end{tikzpicture}
\caption{}
\label{BSC}
\end{subfigure}
%%%%%%%%%%%%%%%%   AsymC for receiving observations    %%%%%%%%%
\hspace{0.03\linewidth}
\begin{subfigure}{0.46\linewidth}
\centering
\begin{tikzpicture}[scale=1.4]
%\begin{scope}[shift={(2.6,0)}]
\draw [decoration={markings,mark=at position 1 with {\arrow[scale=2,>=stealth]{>}}},postaction={decorate}] (0,0) -- (1.5,0);
\draw [decoration={markings,mark=at position 1 with {\arrow[scale=2,>=stealth]{>}}},postaction={decorate}] (0,-1) -- (1.5,-1);
%\draw [decoration={markings,mark=at position 1 with {\arrow[scale=2,>=stealth]{>}}},postaction={decorate}] (0,0) -- (1.5,-1);
\draw [decoration={markings,mark=at position 1 with {\arrow[scale=2,>=stealth]{>}}},postaction={decorate}] (0,-1) -- (1.5,0);
\node at (1.65,0) {$Y$};
\node at (1.65,-1) {$N$};
\node at (-0.15,0) {$Y$};
\node at (-0.15,-1) {$N$};
\node at (-0.35,-0.5) {$A_i$};
\node at (1.85,-0.5) {$O_i$};
\node at (0.75,0.15) {\scalebox{0.9}{$1$}};
\node at (0.75,-1.15) {\scalebox{0.9}{$1-\epsilon$}};
%\node at (0.4,-0.35) [rotate= -26.56] {$1-p$};
%\node at (0.5,-0.19) [rotate= -33.7] {\scalebox{0.9}{$1-p$}};
\node at (0.8,-0.6) [rotate= 33.7] {\scalebox{0.9}{$\epsilon$}};
%\end{scope}
\end{tikzpicture}
\caption{}
\label{ASC}
\end{subfigure}
\setlength{\abovecaptionskip}{2pt}
\caption{\small $(a)$ The BSC through which agents receive private signals. $(b)$ The channel through which agents' actions are corrupted.}
\end{figure}
